Wild Networks: Exposure of 5G Network Infrastructures to Adversarial Examples

Fifth Generation (5G) networks must support billions of heterogeneous devices while guaranteeing optimal Quality of Service (QoS). Such requirements are impossible to meet with human effort alone, and Machine Learning (ML) represents a core asset in 5G. ML, however, is known to be vulnerable to adversarial examples; moreover, as our paper will show, the 5G context is exposed to a yet another type of adversarial ML attacks that cannot be formalized with existing threat models. Proactive assessment of such risks is also challenging due to the lack of ML-powered 5G equipment available for adversarial ML research. To tackle these problems, we propose a novel adversarial ML threat model that is particularly suited to 5G scenarios, and is agnostic to the precise function solved by ML. In contrast to existing ML threat models, our attacks do not require any compromise of the target 5G system while still being viable due to the QoS guarantees and the open nature of 5G networks. Furthermore, we propose an original framework for realistic ML security assessments based on public data. We proactively evaluate our threat model on 6 applications of ML envisioned in 5G. Our attacks affect both the training and the inference stages, can degrade the performance of state-of-the-art ML systems, and have a lower entry barrier than previous attacks.

==> sections/acronym_table.tex <==
\begin{table}[!htbp]
    \centering
    \caption{List of acronyms used in this paper.}
    \label{tab:acronym}
    \resizebox{0.9\columnwidth}{!}{
        \begin{tabular}{|c|c|}
             \hline
             \textbf{Acronym} & \textbf{Meaning} \\
             \hline \hline
             MAC & Medium Access Control \\ \hline
             RRC & Radio Resource Control \\ \hline
             PDCP & Packet Data Convergence Protocol \\ \hline
             ML & Machine Learning \\ \hline
             RAN & Radio Access Network \\ \hline
             gNB & 5G NodeB \\ \hline
             UE & User Equipment \\ \hline
             QoS & Quality of Service \\ \hline
             QoE & Quality of Experience \\ \hline
             CNN & Convolutional Neural Network \\ \hline
             PSNR & Peak Signal to Noise Ratio \\ \hline
             MOS & Mean Opinion Score \\ \hline
             OS & Operating System \\ \hline
             eMBB & enhanced Mobile Broadband \\ \hline
             MMTC & massive Mobile Type Communications \\ \hline
             URLLC & Ultra Reliable and Low Latency Communications \\ \hline
             CQI & Channel Quality Indicator \\ \hline
             SNR & Signal-to-Noise Ratio \\ \hline
             RSSI & Received Signal Strength Indicator \\ \hline
             RSRP & Reference Signal Received Power \\ \hline
             RSRQ & Ratio between RSRP and RSSI \\ \hline
             AMR & Automatic Modulation Recognition \\ \hline
             IANA & Internet Assigned Numbers Association \\ \hline
             DU & Distributed Units \\ \hline
             CU & Centralized Units \\ \hline
             SLA & Service Level Agreement \\ \hline
             CPU & Central Processing Unit \\ \hline
             NIST & National Institute of Standards and Technology \\ \hline
             APT & Advanced Persistent Threat \\ \hline
             CS & Case Studies \\ \hline
             KPI & Key Performance Indicators \\ \hline
             OSINT & Open Source INTelligence \\ \hline
             
             
             
        \end{tabular}
    }
\end{table}
